Learning Video Object Segmentation from Static Images

Inspired by recent advances of deep learning in instance segmentation and object tracking, we introduce video object segmentation problem as a concept of guided instance segmentation. Our model proceeds on a per-frame basis, guided by the output of the previous frame towards the object of interest in the next frame. We demonstrate that highly accurate object segmentation in videos can be enabled by using a convnet trained with static images only. The key ingredient of our approach is a combination of offline and online learning strategies, where the former serves to produce a refined mask from the previous frame estimate and the latter allows to capture the appearance of the specific object instance. Our method can handle different types of input annotations: bounding boxes and segments, as well as incorporate multiple annotated frames, making the system suitable for diverse applications. We obtain competitive results on three different datasets, independently from the type of input annotation.

==> sup_material/sections/attribute_analysis.tex <==
\section{Attribute-based evaluation}
\label{sec:attr_eval}

Table \ref{tab:attr-eval} presents a more detailed evaluation on DAVIS using video attributes and complements Figure 5 in the main paper. 

The attribute based evaluation shows that our generic model, $\mathtt{MaskTrack}$, 
is robust to various video challenges present in DAVIS. It compares favourably on any subset of videos sharing the same attribute, except camera-shake, where $\mathtt{ObjFlow}$ \cite{Tsai2016Cvpr} marginally outperforms our approach.

We observe that $\mathtt{MaskTrack}$ handles well fast-motion, appearance change and out-of-view, where competitive methods are failing \cite{Maerki2016Cvpr, Tsai2016Cvpr}.\\
Furthermore, incorporating optical flow information and CRF post-processing into $\mathtt{MaskTrack}$ substantially increases robustness on all categories, reaching over 70$\%$ mIoU on each subcategory.
In particular, $\mathtt{MaskTrack\mathsmaller{+}Flow \mathsmaller{+}CRF}$
better discriminates cases of low resolution, scale-variation and appearance change. 

\begin{table*}
\begin{centering}
\begingroup
%\setlength{\tabcolsep}{0.15em}
\begin{tabular}{l|ccc||cc}
% \hline
\multirow{2}{*}{Attribute} & \multicolumn{5}{c}{Method, mIoU}\\
& $\mathtt{BVS}$ \cite{Maerki2016Cvpr} & $\mathtt{ObjFlow}$ \cite{Tsai2016Cvpr}& $\mathtt{MaskTrack}$ & $\mathtt{MaskTrack\mathsmaller{+}Flow}$ & $\mathtt{MaskTrack\mathsmaller{+}Flow \mathsmaller{+}CRF}$\tabularnewline
\hline
\hline
Appearance change & 0.46& 0.54& \textbf{0.65} & 0.75& 0.76\tabularnewline
Fast-motion & 0.53 & 0.55& \textbf{0.66} & 0.74 & 0.75\tabularnewline
Background clutter& 0.63 & 0.68 & \textbf{0.77} & 0.78 & 0.79\tabularnewline
Camera-shake& 0.62 & \textbf{0.72} & 0.71 & 0.77 & 0.78\tabularnewline
Dynamic background& 0.6 & 0.67 & \textbf{0.69}& 0.75 & 0.76\tabularnewline
Deformation& 0.7& 0.77& \textbf{0.77} &0.78 & 0.8\tabularnewline
Edge ambiguity& 0.58 & 0.65& \textbf{0.68} & 0.74 & 0.74\tabularnewline
Heterogeneous object& 0.63 & 0.66 & \textbf{0.71} & 0.77 &0.79\tabularnewline
Interacting objects& 0.63 & 0.68 & \textbf{0.74} & 0.75 &0.77\tabularnewline
Low resolution& 0.59& 0.58& \textbf{0.6} & 0.75 & 0.77\tabularnewline
Motion blur& 0.58& 0.6& \textbf{0.66}& 0.72 & 0.74\tabularnewline
Occlusion& 0.68 & 0.66 & \textbf{0.74} & 0.75 & 0.77\tabularnewline
Out-of-view& 0.43 & 0.53 & \textbf{0.66} & 0.71 & 0.71\tabularnewline
Scale variation& 0.49 & 0.56 & \textbf{0.62}& 0.72 & 0.73\tabularnewline
Shape complexity& 0.67 & 0.69 & \textbf{0.71} & 0.72 & 0.75\tabularnewline
% \hline
\end{tabular}\endgroup
\par\end{centering}
\caption{\label{tab:attr-eval}Attribute based evaluation on DAVIS.}
\end{table*}


==> sup_material/sections/content.tex <==
\section{Content}
\label{sec:content}

This supplementary material provides both additional
quantitative and qualitative results, as well as an attached
video. 

\begin{itemize}

\item Section \ref{sec:add_res} provides additional quantitative results for DAVIS, YoutubeObjects, and SegTrackv-2 (see Tables \ref{tab:youtube_cat} - \ref{tab:segtrack_seq}).
\item Additional qualitative results with first frame box and segment supervision are presented in Section \ref{sec:add_qual_res} and Figure \ref{fig:qualitative-results}.
\item Detailed attribute-based evaluation is reported in Section \ref{sec:attr_eval} and Table \ref{tab:attr-eval}.
\item Examples of mask generation for the extra input channel are shown in Section \ref{sec:mask_gen} and Figure \ref{fig:offline-augmentation}.
\item The dataset specific tuning for additional ingredients is described in Section \ref{sec:dat_tun}.
\item Examples of optical flow magnitude images are presented in Section \ref{sec:flow_gen} and Figure \ref{fig:flow_images}.
\item Instructions to see the video are detailed in Section \ref{sec:video_codec}.

% \item Explain strategy for CRF per-dataset tuning <- To be drafted by Federico
% 
% \item Additional qualitative images of flow magnitude, for all three datasets
% 
% % \item Show baseline quantile curves for multiple frame annotations analysis (and repeat the ones in figure 7). Add a bit of blabhblhah analysis.
% 
% \item More examples of figure 2 (mask generation)

\end{itemize}

\begin{comment}

Ideas for the video:

- What does it take to be at https://www.youtube.com/user/DisneyResearchHub

- Self contained presentation (ready to go to youtube)

- Couple of slides to explain (high level) the method (use figure 1, and wording from paper)

- Couple of examples of our method (alone)

- Couple of examples comparing to other methods

- Couple of examples showing how adding flow further help (flow/no-flow). Show failure cases of MaskTrack where MaskTrack+flow+crf helps.

- More, more examples of MaskTrack+flow+crf versus others

-> Target ~4 minutes video

\end{comment}


\begin{comment}

Releases:

- Full Code ?
- Test time code only ?
- Models (and "demo test time") ?  (note that if test time code is not in full, then 50 models for Davis)
- Result masks for all experiments in table 2 and Mastrack+flow+crf on Davis ?


\end{comment}



==> sup_material/sections/results.tex <==
\section{Additional quantitative results}
\label{sec:add_res}
In this section we present additional quantitative results for three different datasets: DAVIS \cite{Perazzi2016Cvpr}, YoutubeObjects \cite{Prest2012Cvpr}, and SegTrackv-2  \cite{Li2013Iccv}.
This section complements Section 5.3 in the main paper.

\paragraph{YoutubeObjects}
The per-category comparison with other state-of-the-art methods on YoutubeObjects is shown in Table \ref{tab:youtube_cat}.

\begin{table}
\begin{centering}
\begingroup
%\setlength{\tabcolsep}{0.15em}
\begin{tabular}{l@{   }|@{   }c@{   }c@{   }c@{   }}
% \hline
\multirow{2}{*}{Category} & \multicolumn{3}{c}{Method, mIoU}\\
& $\mathtt{BVS}$ \cite{Maerki2016Cvpr} & $\mathtt{ObjFlow}$ \cite{Tsai2016Cvpr}& $\mathtt{MaskTrack}$ \tabularnewline
\hline
\hline
aeroplane& 80.8& \textbf{85.3} & 81.6\tabularnewline
bird & 76.4 & \textbf{83.1}& 82.9 \tabularnewline
boat& 60.1 & 70.6 & \textbf{74.7} \tabularnewline
car& 56.7 & \textbf{68.8} & 66.9 \tabularnewline
cat& 52.7 & 60.6 & \textbf{69.6}\tabularnewline
cow& 64.8& 71.5 & \textbf{75.0} \tabularnewline
dog& 61.6 & 71.6 & \textbf{75.2} \tabularnewline
horse& 53.1 & 62.3 & \textbf{64.9} \tabularnewline
motorbike& 41.6 & \textbf{59.9} & 49.8 \tabularnewline
train& 62.1& 74.7 & \textbf{77.7} \tabularnewline
\hline
Mean per object& 59.7 & 70.1 & \textbf{71.7} \tabularnewline
Mean per class& 61.0 & 70.9 & \textbf{71.9} \tabularnewline
% \hline
\end{tabular}\endgroup
\par\end{centering}
\caption{\label{tab:youtube_cat}Per-category results on the YoutubeObjects dataset.}
\end{table}

\paragraph{DAVIS}

We present the per-sequence comparison with other state-of-the-art methods on DAVIS in Table \ref{tab:davis_seq}.

\paragraph{SegTrack-v2}

Table \ref{tab:segtrack_seq} reports the per-sequence comparison with other state-of-the-art methods on SegTrack-v2.



\begin{table}
\begin{centering}
\begingroup
%\setlength{\tabcolsep}{0.15em}
\begin{tabular}{l|@{   }c@{   }c@{   }c@{   }}
% \hline
\multirow{2}{*}{Sequence} & \multicolumn{3}{c}{Method, mIoU}\\
& $\mathtt{BVS}$ \cite{Maerki2016Cvpr} & $\mathtt{ObjFlow}$ \cite{Tsai2016Cvpr}& $\mathtt{MaskTrack}$ \tabularnewline
\hline
\hline
bear                & \bf 95.5    &     94.6    &     92.8    \\
car-shadow          &     57.8    &     84.6    & \bf 90.3    \\
elephant            &     84.9    &     87.9    & \bf 91.4    \\
lucia               & \bf 90.1    &     89.7    &     88.4    \\
rollerblade         &     58.8    & \bf 88.6    &     33.0    \\
blackswan           &     94.3    & \bf 94.7    &     91.9    \\
car-turn            &     84.4    &     87.6    & \bf 92.3    \\
flamingo            & \bf 88.1    &     87.3    &     70.9    \\
mallard-fly         & \bf 60.6    &     55.0    &     56.7    \\
scooter-black       &     33.7    & \bf 76.5    &     64.9    \\
bmx-bumps           &     43.4    & \bf 48.0    &     39.6    \\
cows                &     89.5    &     91.0    & \bf 91.9    \\
goat                &     66.1    & \bf 86.5    &     85.8    \\
mallard-water       &     90.7    &     89.9    & \bf 91.0    \\
scooter-gray        &     50.8    &     29.6    & \bf 81.7    \\
bmx-trees           & \bf 38.2    &     14.9    &     32.1    \\
dance-jump          &     74.5    & \bf 80.4    &     66.2    \\
hike                &     75.5    & \bf 93.4    &     74.5    \\
motocross-bumps     &     40.1    &     48.5    & \bf 53.9    \\
soapbox             &     78.9    &     68.9    & \bf 86.1    \\
boat                &     64.4    & \bf 80.8    &     78.2    \\
dance-twirl         &     49.2    &     56.7    & \bf 67.8    \\
hockey              &     82.9    & \bf 85.0    &     84.0    \\
motocross-jump      &     34.1    &     59.4    & \bf 69.0    \\
soccerball          &     84.4    &     8.0     & \bf 85.8    \\
breakdance          &     50.0    &     49.6    & \bf 59.4    \\
dog                 &     72.3    & \bf 89.7    &     86.8    \\
horsejump-high      &     80.1    & \bf 86.2    &     78.4    \\
motorbike           & \bf 56.3    &     47.8    &     46.5    \\
stroller            &     76.7    & \bf 87.7    &     86.2    \\
breakdance-flare    &     72.7    &     76.5    & \bf 89.2    \\
dog-agility         &     34.5    & \bf 86.0    &     83.7    \\
horsejump-low       &     60.1    & \bf 82.2    &     79.6    \\
paragliding         &     87.5    & \bf 94.7    &     93.2    \\
surf                &     49.2    & \bf 95.6    &     92.6    \\
bus                 & \bf 86.3    &     68.2    &     79.1    \\
drift-chicane       &     3.3     & \bf 17.5    &     0.5     \\
kite-surf           &     42.5    & \bf 70.2    &     58.7    \\
paragliding-launch  & \bf 64.0    &     63.7    &     58.9    \\
swing               &     78.4    &     60.4    & \bf 80.7    \\
camel               &     66.9    & \bf 86.7    &     80.4    \\
drift-straight      &     40.2    &     31.4    & \bf 46.0    \\
kite-walk           & \bf 87.0    &     85.0    &     77.4    \\
parkour             &     75.6    & \bf 86.1    &     85.3    \\
tennis              &     73.7    &     81.8    & \bf 87.3    \\
car-roundabout      &     85.1    & \bf 90.0    &     82.8    \\
drift-turn          &     29.9    &     3.5     & \bf 86.5    \\
libby               &     77.6    &     59.4    & \bf 78.8    \\
rhino               &     78.2    &     89.5    & \bf 93.2    \\
train               &     87.2    & \bf 91.7    &     90.8    \\
\hline
Mean                &  66.5   &    71.1   &  \bf 74.8   \\
% \hline
\end{tabular}\endgroup
\par\end{centering}
\caption{\label{tab:davis_seq}Per-sequence results on the DAVIS dataset.}
\end{table}

\begin{table}
\begin{centering}
\begingroup
%\setlength{\tabcolsep}{0.15em}
\begin{tabular}{l@{  }|@{   }c@{   }c@{   }c@{   }c@{   }}
% \hline
\multirow{2}{*}{Sequence} & \multicolumn{4}{c}{Method, mIoU}\\
& $\mathtt{BVS}$ \cite{Maerki2016Cvpr} & $\mathtt{ObjFlow}$ \cite{Tsai2016Cvpr}& $\mathtt{TRS}$ \cite{Xiao2016Cvpr} & $\mathtt{MaskTrack}$ \tabularnewline
\hline
\hline
bird of paradise & 89.7 & 87.1 & \bf 90.0 &84.0 \\
birdfall & 65.3 & 52.9 &  \bf 72.5& 56.6 \\
bmx\#1 & 67.1 &  \bf 87.9 & 86.1 &81.9 \\
bmx\#2 & 3.2 & 4.0 & \bf  40.3 & 0.1 \\
cheetah\#1 & 5.4 & 25.9 & 61.2 &  \bf 69.3 \\
cheetah\#2 & 9.2 & 37.2 &  \bf 39.4 & 17.4 \\
drift\#1 & 68.5 & \bf  77.9 & 70.7 & 47.4 \\
drift\#2 & 32.7 & 27.4 & 70.7 &  \bf 70.9 \\
frog & 76.1 & 78.4 & 80.2 &  \bf  85.3 \\
girl & 86.5 & 84.2 & 86.4 &  \bf 86.8 \\
hummingbird\#1 & 53.2 & \bf  67.2 & 53.0 & 39.0 \\
hummingbird\#2 & 28.7 & 68.5 &  \bf 70.5 & 49.6 \\
monkey & 85.7 & 87.8 & 83.1 &  \bf 89.3 \\
monkeydog\#1 & 40.5 & 47.1 &  \bf 74.0 & 25.3 \\
monkeydog\#2 & 17.1 & 21.0 &  \bf 39.6 & 31.7 \\
parachute & 93.7 & 93.3 &  \bf 95.9 & 93.7 \\
penguin\#1 & 81.6 & 80.4 & 53.2 &  \bf 93.7 \\
penguin\#2 & 82.0 & 83.5 & 72.9 &  \bf 85.2 \\
penguin\#3 & 78.5 & 83.9 & 74.4 &  \bf 90.1 \\
penguin\#4 & 76.4 & 86.2 & 57.2 & \bf  90.5 \\
penguin\#5 & 47.8 &  \bf 82.3 & 63.5 & 78.4 \\
penguin\#6 & 84.3 & 87.3 & 65.7 &  \bf 89.3 \\
soldier & 55.3 & \bf  86.8 & 76.3 & 82.0 \\
worm & 65.4 & 83.2 & \bf  82.4 &80.4 \\
\hline
Mean  &  58.4   &     67.5  & \bf 69.1 & 67.4   \\
% \hline
\end{tabular}\endgroup
\par\end{centering}
\caption{\label{tab:segtrack_seq}Per-sequence results on the SegTrack-v2 dataset.}
\end{table}


\section{Additional qualitative results}
\label{sec:add_qual_res}

In this section we provide additional qualitative results for the $\mathtt{MaskTrack}_{Box}$ and $\mathtt{MaskTrack}$ systems, described in Section 3 in the man paper.
Figure \ref{fig:qualitative-results} shows the video object segmentation results when considering different types of annotations on DAVIS. Starting from segment annotations or even only from box annotations
on the first frame, our model generates high quality segmentations, making the system suitable for diverse applications.

\begin{figure*}
\begin{centering}
\setlength{\tabcolsep}{1pt}
\begin{tabular}{ccccccc}

\begin{turn}{90}
{\footnotesize{\hspace{1em} Box}}
\end{turn} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/rhino1_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/rhino10_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/rhino30_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/rhino50_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/rhino65_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/rhino89_box.jpg} \tabularnewline
\begin{turn}{90}
{\footnotesize{\hspace{0.5em} Segment}}
\end{turn}  &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/rhino1_gt.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/rhino10_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/rhino30_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/rhino50_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/rhino65_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/rhino89_segment.jpg} \tabularnewline
\\

\begin{turn}{90}
{\footnotesize{\hspace{1em} Box}}
\end{turn} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/stroller1_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/stroller10_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/stroller30_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/stroller50_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/stroller65_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/stroller89_box.jpg} \tabularnewline
\begin{turn}{90}
{\footnotesize{\hspace{0.5em} Segment}}
\end{turn}  &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/stroller1_gt.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/stroller10_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/stroller30_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/stroller50_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/stroller65_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/stroller89_segment.jpg} \tabularnewline

\\

\begin{turn}{90}
{\footnotesize{\hspace{1em} Box}}
\end{turn} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/car1_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/car10_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/car30_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/car50_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/car65_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/car89_box.jpg} \tabularnewline
\begin{turn}{90}
{\footnotesize{\hspace{0.5em} Segment}}
\end{turn}  &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/car1_gt.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/car10_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/car30_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/car50_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/car65_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/car89_segment.jpg} \tabularnewline

\\

\begin{turn}{90}
{\footnotesize{\hspace{1em} Box}}
\end{turn} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/hockey1_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/hockey10_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/hockey30_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/hockey50_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/hockey65_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/hockey89_box.jpg} \tabularnewline
\begin{turn}{90}
{\footnotesize{\hspace{0.5em} Segment}}
\end{turn}  &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/hockey1_gt.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/hockey10_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/hockey30_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/hockey50_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/hockey65_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/hockey89_segment.jpg} \tabularnewline

\\

\begin{turn}{90}
{\footnotesize{\hspace{1em} Box}}
\end{turn} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/boat1_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/boat10_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/boat30_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/boat50_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/boat65_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/boat89_box.jpg} \tabularnewline
\begin{turn}{90}
{\footnotesize{\hspace{0.5em} Segment}}
\end{turn}  &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/boat1_gt.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/boat10_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/boat30_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/boat50_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/boat65_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/boat89_segment.jpg} \tabularnewline

\\

\begin{turn}{90}
{\footnotesize{\hspace{1em} Box}}
\end{turn} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/duck1_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/duck10_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/duck30_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/duck50_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/duck65_box.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/duck89_box.jpg} \tabularnewline
\begin{turn}{90}
{\footnotesize{\hspace{0.5em} Segment}}
\end{turn}  &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/duck1_gt.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/duck10_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/duck30_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/duck50_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/duck65_segment.jpg} &
\includegraphics[width=0.16\textwidth,height=0.06\textheight]{figures/annot_results/duck89_segment.jpg} \tabularnewline


&\footnotesize{}1st frame annotation & \multicolumn{5}{c}{\footnotesize{} Results with $\mathtt{MaskTrack}_{Box}$ and $\mathtt{MaskTrack}$, the frames are chosen equally distant based on the video sequence length}
\end{tabular}
\par\end{centering}
\caption{\label{fig:qualitative-results}
Qualitative results of  $\mathtt{MaskTrack}_{Box}$ and $\mathtt{MaskTrack}$ on Davis using 1st frame annotation supervision (box or segment).
By propagating annotation from the 1st frame, either from segment or just bounding box annotations, our system generates results comparable to ground truth.}
\end{figure*}

\input{sup_material/sections/attribute_analysis.tex}

\section{Examples of training mask generation}
\label{sec:mask_gen}

In Section 5.2 of the main paper we show that the main factor affecting the quality is using any form of mask deformations when creating the training samples (both for offline and online training).
The mask deformation ingredient is crucial for our $\mathtt{MaskTrack}$ approach, making the segmentation estimation more robust at test time to the noise in the input mask.
Figure \ref{fig:offline-augmentation} complements Figure 2 in the main paper and shows examples of generated masks using affine transformation as well as non-rigid deformations via thin-plate splines
(see Section 4 in the main paper for more details).



\begin{figure*}[t]
\begin{centering}
\begin{tabular}{@{}cc@{ }c@{ }c@{ }c@{ }c@{}}
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/blackswan_gt.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/blackswan_jit_1.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/blackswan_jit_2.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/blackswan_jit_3.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/blackswan_jit_4.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/blackswan_jit_5.jpg} \\

\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/rhino_gt.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/rhino_jit_1.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/rhino_jit_2.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/rhino_jit_3.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/rhino_jit_4.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/rhino_jit_5.jpg} \\

\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/libby_gt.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/libby_jit_1.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/libby_jit_2.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/libby_jit_3.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/libby_jit_4.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/libby_jit_5.jpg} \\

\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/hockey_gt.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/hockey_jit_1.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/hockey_jit_2.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/hockey_jit_3.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/hockey_jit_4.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/hockey_jit_5.jpg} \\

\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/elephant_gt.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/elephant_jit_1.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/elephant_jit_2.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/elephant_jit_3.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/elephant_jit_4.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/elephant_jit_5.jpg} \\

\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/breakdance-flare_gt.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/breakdance-flare_jit_1.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/breakdance-flare_jit_2.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/breakdance-flare_jit_3.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/breakdance-flare_jit_4.jpg} &
\includegraphics[width=0.16\textwidth,height=0.08\textheight]{figures/masks_deform/breakdance-flare_jit_5.jpg} \\
Annotated image & \multicolumn{5}{c}{Example training masks}\\
\end{tabular}
\par\end{centering}
\caption{\label{fig:offline-augmentation}Examples of training mask generation.
From one annotated image, multiple training masks are generated. The generated masks mimic plausible object shapes on the preceding frame.
}
\vspace{-1em}
\end{figure*}

\section{Dataset specific tuning}
\label{sec:dat_tun}
As mentioned in Section 5.3 in the main paper by adding additional ingredients specifically tuned for
different datasets, such as optical flow and CRF post-processing, we can push the results even further, reaching
80.0 mIoU on DAVIS, 72.6 on YoutubeObjects and 70.3 on SegTrackv-2.
In this section we discuss the dataset specific tuning.

\paragraph{Optical flow}
Although optical flow can provide interesting gains, we
found it to be brittle when going across different datasets.
Therefore we explored different strategies to handle optical flow.

As discussed in Section 3.3 of the main paper
given a video sequence, we compute the optical flow using EpicFlow \cite{EpicFlowCVPR15} with Flow Fields matches \cite{FlowFields15} and convolutional boundaries \cite{COB_Maninis16}.
In parallel to the $\mathtt{MaskTrack}$ with RGB images, we proceed to compute a second output mask using the magnitude of the optical flow field as input image (replicated into a three channel image).
We then fuse by averaging the output scores given by the two parallel networks (using RGB image and optical flow magnitude as inputs).

For DAVIS  we use the original $\mathtt{MaskTrack}$ model (trained with RGB images) as-is, without retraining. However, this strategy fails on YoutubeObjects and SegTrackv-2, mainly due to the failure modes of the optical flow
algorithm and its sensitivity to the video data quality. To overcome this limitation we additionally trained the $\mathtt{MaskTrack}$ model using optical flow magnitude images on video data instead of RGB images.
Training on optical flow magnitude images helps the network to be robust to the optical flow errors during the test time and provides a marginal improvement on YoutubeObjects and SegTrackv-2.

Overall integrating optical flow on top of $\mathtt{MaskTrack}$ provides $1\negmedspace\sim\negmedspace4 \%$ on each dataset.

\paragraph{CRF post-processing}
As have been shown in \cite{Chen2016ArxivDeeplabv2} adding on top a well-tuned post-processing CRF \cite{Kraehenbuehl2011Nips} can gain a
couple of mIoU points. Therefore following \cite{Chen2016ArxivDeeplabv2} we cross-validate the parameters of the fully connected CRF per each dataset based on the available first frame segment annotations of all video sequences.
We employ coarse-to-fine search scheme for tuning CRF parameters and fix the number of mean field iterations to 10. We apply the CRF on a temporal window of 3 frames to improve the temporal stability of the results. The color (RGB) and the spatio-temporal (XYT) standard deviation of the \emph{appearance kernel} are set, respectively, to 10 and 5. The pairwise term weight is set to 5. We employ an additional \emph{smoothness kernel} to remove small isolated regions. Both its weight and the spatial (XY) standard deviation are set to 1.

\section{Examples of optical flow magnitude images}
\label{sec:flow_gen}

Section 3.3 in the main paper proposes to employ optical flow magnitude as a source of additional information to guide the segmentation.
The flow magnitude roughly looks like a gray-scale object and captures useful object shape information, therefore complementing the $\mathtt{MaskTrack}$ model with RGB images as inputs.
Examples of optical flow magnitude images are shown in Figure \ref{fig:flow_images} for three different datasets. Figure \ref{fig:flow_images} complements Figure 3 in the main paper.
\begin{figure*}
% General space between cols (6pt standard)
\begin{centering}
% \hspace*{\fill}
\begin{centering}
\begin{tabular}{@{}c@{  }c@{  }c@{  }c@{  }c@{}}
%& Boxes & Segments\\


&\multicolumn{4}{c}{\bf DAVIS} \tabularnewline
\\
\begin{turn}{90}{\hspace{0.5em} RGB Image}
\end{turn}
&\includegraphics[width=0.24\textwidth,height=0.11\textheight]{figures/flow_images/image_boat_00003.jpg} &
\includegraphics[width=0.24\textwidth,height=0.11\textheight] {figures/flow_images/image_dance_jump_00015.jpg} &
\includegraphics[width=0.24\textwidth,height=0.11\textheight] {figures/flow_images/image_horse_00005.jpg}&
\includegraphics[width=0.24\textwidth,height=0.11\textheight] {figures/flow_images/image_goat_00077.jpg} \tabularnewline
%&\multicolumn{4}{c}{\footnotesize{} RGB image} \tabularnewline
\begin{turn}{90}
{\hspace{0.5em} Optical Flow}
\end{turn}
&\includegraphics[width=0.24\textwidth,height=0.11\textheight]{figures/flow_images/boat_00003.jpg} &
\includegraphics[width=0.24\textwidth,height=0.11\textheight] {figures/flow_images/dance_jump_00015.jpg} &
\includegraphics[width=0.24\textwidth,height=0.11\textheight] {figures/flow_images/horse_00005.jpg}&
\includegraphics[width=0.24\textwidth,height=0.11\textheight] {figures/flow_images/goat_00077.jpg} \tabularnewline
%&\multicolumn{4}{c}{\footnotesize{} Optical flow magnitude} \tabularnewline
\\
\\
&\multicolumn{4}{c}{\bf YoutubeObjects} \tabularnewline
\\
\begin{turn}{90}{\hspace{0.5em} RGB Image}
\end{turn}
&\includegraphics[width=0.24\textwidth,height=0.11\textheight]{figures/flow_images/image_aeroplane_frame0114.jpg} &
\includegraphics[width=0.24\textwidth,height=0.11\textheight] {figures/flow_images/image_cat_frame0203.jpg} &
\includegraphics[width=0.24\textwidth,height=0.11\textheight] {figures/flow_images/image_frame0063.jpg}&
\includegraphics[width=0.24\textwidth,height=0.11\textheight] {figures/flow_images/image_bird_frame0107.jpg} \tabularnewline
%&\multicolumn{4}{c}{\footnotesize{} RGB image} \tabularnewline
\begin{turn}{90}
{\hspace{0.5em} Optical Flow}
\end{turn}
&\includegraphics[width=0.24\textwidth,height=0.11\textheight]{figures/flow_images/aeroplane_frame0114.jpg} &
\includegraphics[width=0.24\textwidth,height=0.11\textheight] {figures/flow_images/cat_frame0203.jpg} &
\includegraphics[width=0.24\textwidth,height=0.11\textheight] {figures/flow_images/motorbike_frame0063.jpg}&
\includegraphics[width=0.24\textwidth,height=0.11\textheight] {figures/flow_images/bird_frame0107.jpg} \tabularnewline
%&\multicolumn{4}{c}{\footnotesize{} Optical flow magnitude} \tabularnewline
\\
\\
&\multicolumn{4}{c}{\bf SegTrack-v2} \tabularnewline
\\
\begin{turn}{90}{\hspace{0.5em} RGB Image}
\end{turn}
&\includegraphics[width=0.24\textwidth,height=0.11\textheight]{figures/flow_images/image_bmx_06703.jpg} &
\includegraphics[width=0.24\textwidth,height=0.11\textheight] {figures/flow_images/image_frog_0000000161.jpg} &
\includegraphics[width=0.24\textwidth,height=0.11\textheight] {figures/flow_images/image_monkey_0000000002.jpg}&
\includegraphics[width=0.24\textwidth,height=0.11\textheight] {figures/flow_images/image_soldier_011.jpg} \tabularnewline
%&\multicolumn{4}{c}{\footnotesize{} RGB image} \tabularnewline
\begin{turn}{90}
{\hspace{0.5em} Optical Flow}
\end{turn}
&\includegraphics[width=0.24\textwidth,height=0.11\textheight]{figures/flow_images/bmx_06703.jpg} &
\includegraphics[width=0.24\textwidth,height=0.11\textheight] {figures/flow_images/frog_0000000161.jpg} &
\includegraphics[width=0.24\textwidth,height=0.11\textheight] {figures/flow_images/monkey_0000000002.jpg}&
\includegraphics[width=0.24\textwidth,height=0.11\textheight] {figures/flow_images/soldier_011.jpg} \tabularnewline
%&\multicolumn{4}{c}{\footnotesize{} Optical flow magnitude} \tabularnewline
\end{tabular}
\par\end{centering}

\par\end{centering}
\caption{\label{fig:flow_images}Examples of optical flow magnitude images for three different datasets.}
\end{figure*}




==> sup_material/sections/video_codec.tex <==
\section{Video codec}
\label{sec:video_codec}

The attached video is encoded with Xvid MPEG-4. We
tested opening the video with: \textbf{Mac}: VLC Player (\url{http://www.videolan.org/vlc/}, works also for Windows/Linux). \textbf{Windows}: Windows media player. \textbf{Linux}: mplayer.
For windows, a compatible codec is available at \url{http://www.codecguide.com/download_kl.htm}.
